A Rusty Link in the AI Supply Chain: Detecting Evil Configurations in Model Repositories

Recent advancements in large language models (LLMs) have spurred the development of diverse AI applications from code generation and video editing to text generation; however, AI supply chains such as Hugging Face, which host pretrained models and their associated configuration files contributed by the public, face significant security challenges; in particular, configuration files originally intended to set up models by specifying parameters and initial settings can be exploited to execute unauthorized code, yet research has largely overlooked their security compared to that of the models themselves; in this work, we present the first comprehensive study of malicious configurations on Hugging Face, identifying three attack scenarios (file, website, and repository operations) that expose inherent risks; to address these threats, we introduce CONFIGSCAN, an LLM-based tool that analyzes configuration files in the context of their associated runtime code and critical libraries, effectively detecting suspicious elements with low false positive rates and high accuracy; our extensive evaluation uncovers thousands of suspicious repositories and configuration files, underscoring the urgent need for enhanced security validation in AI model hosting platforms.

==> algorithms/overview2.tex <==
\begin{algorithm}
\caption{ConfigScan}
\label{alg:ConfigScan}
\begin{algorithmic}[1]
\State \textbf{Input:} README FILE $R$, CONFIG FILE $C$, Vulnerability LLM $VLLM$ and Score LLM $SLLM$
\State \textbf{Output:} Vulnerability $\mathbb{V}$, POC $\mathbb{P}$, Confidence Score $S$, Process of Analysis $\mathbb{A}$
\State $\mathbb{K_f} = Json\_Data\_Parsing(C) $
\State $\mathbb{K_R} = README\_Summarization(R)$ 
\State $\mathbb{V}, \mathbb{P}, \mathbb{A} = VLLM(K_f, K_R, C)$
\State $S = SLLM(\mathbb{V}, \mathbb{P}, \mathbb{A}, C)$
\If{$S>0 \&\& S<1$}
$S_Pre=S$
\State INT COUNT=0
\For{$V$ in $\mathbb{V}$}
\For{$i < N$}
\State $\mathbb{V}, \mathbb{P}, \mathbb{A} = VLLM(K_f, K_R, C, V)$
\State $S_L = SLLM(\mathbb{V}, \mathbb{P}, \mathbb{A}, C, V)$
\If {$S_L>S_{Pre}$}
\State $S_{Pre}=S_L$
\State $COUNT+=1$
\If {$COUNT>n$}
\State return $\mathbb{V}, \mathbb{P}, \mathbb{A}, C$
\EndIf
\EndIf
\EndFor
\EndFor
\EndIf
\State return $\mathbb{V}, \mathbb{P}, \mathbb{A}, C$
\end{algorithmic}
\end{algorithm}

==> discussion.tex <==
\section{Limitations}
\noindent \textbf{Limited Dataset Scope.} Due to API constraints and time limitations, our analysis was conducted on 1,000 samples of  repositories rather than the entire set. Although this subset provides meaningful insights, a more comprehensive study using a larger dataset is needed to validate the generalizability of our tool.

\noindent \textbf{Focus on JSON Files.} This paper primarily focuses on analyzing JSON configuration files, as they are widely used on platforms like Hugging Face. However, many repositories also use YAML and other formats for configuration. While our approach can be extended to YAML files, further validation is necessary to evaluate its effectiveness across different formats.

==> table/table2.tex <==
\begin{table}[t]
    \caption{Rule-based ConfigScan Analysis}
    \label{tab:rule} 
    \centering
    \tabcolsep=4.5pt
    \resizebox{\linewidth}{!}{ % Resize to fit single column
    \begin{tabular}{lcc}
        \toprule
        \textbf{Potential Risk} & \textbf{Suspicious Repositories} & \textbf{Suspicious Config Files} \\ 
        \midrule
        File Operation Risk  & 13,091  & 13,091 \\ 
        Website Operation Risk  & 1,324  & 1,215 \\ 
        Repository Operation Risk  & 35,761  & 31,373 \\ 
        \bottomrule
    \end{tabular}
    }
    \vspace{-2mm}
\end{table}
